Scaling up Copy Detection

Recent research shows that copying is prevalent for Deep-Web data and considering copying can significantly improve truth finding from conflicting values. However, existing copy detection techniques do not scale for large sizes and numbers of data sources, so truth finding can be slowed down by one to two orders of magnitude compared with the corresponding techniques that do not consider copying. In this paper, we study {\em how to improve scalability of copy detection on structured data}. Our algorithm builds an inverted index for each \emph{shared} value and processes the index entries in decreasing order of how much the shared value can contribute to the conclusion of copying. We show how we use the index to prune the data items we consider for each pair of sources, and to incrementally refine our results in iterative copy detection. We also apply a sampling strategy with which we are able to further reduce copy-detection time while still obtaining very similar results as on the whole data set. Experiments on various real data sets show that our algorithm can reduce the time for copy detection by two to three orders of magnitude; in other words, truth finding can benefit from copy detection with very little overhead.

==> 5_sample.tex <==
\eat{\begin{table}
\centering
{\small
\caption{Summary of representative algorithms.\label{tbl:rep-algorithms}}
\begin{tabular}{|c|c|c|c|c|}
\hline
Methods&Index&Pruning&Incremental&Sampling\\
\hline
{\sc pairwise} & & & & \\
\hline
{\sc pairwise+uniform} & & & &* \\
{\sc basic} & * & & & \\
{\sc hybrid} & * & * &&\\
{\sc incremental} &*&*&*&\\
{\sc incremental +} &\multirow{2}{*}{*}&\multirow{2}{*}{*}&\multirow{2}{*}{*}&\multirow{2}{*}{*}\\
{\sc source-base}&&&&\\

\hline
\end{tabular}}
\end{table}

\begin{figure*}[t]
%\vspace{-.2in}
\begin{minipage}[b]{0.49\textwidth}
\center
\includegraphics[width=3.5in]{figs/overview-efficiency-comp.pdf}
\center

\vspace{-.1in}
{\small (a) Computations.}

\end{minipage}
\begin{minipage}[b]{0.49\textwidth}
%\center
\hspace{.1in}
\includegraphics[width=3.5in]{figs/overview-efficiency-time.pdf}
\center

\vspace{-.1in}
{\small (b) Execution time.}

\end{minipage}

\vspace{-.1in} 
\caption{\small Efficiency overview.\label{fig:overview_efficiency}}
\vspace{-.1in}
\end{figure*}
}

When there are a lot of data items, even with early pruning
we may still need to consider a lot of data items 
for each pair of sources before termination. 
This is because initially both $C_{\to/\leftarrow}^{min}$ 
and $C_{\to/\leftarrow}^{max}$ are functions of the number of shared data items
(\ie, $|\bar D(S_1) \cap \bar D(S_2)|$); the more shared data items,
the smaller $C_{\to/\leftarrow}^{min}$ and the larger $C_{\to/\leftarrow}^{max}$, 
and the longer it can take to terminate. 

One obvious solution to reduce the number of data items is to 
sample a certain percentage of the data items. However, a naive uniform random sampling 
does not work when some sources provide only a small number of
items: we may sample too few data items from such sources
and make wrong decisions.
To solve the problem, we wish to guarantee that from each
source we sample at least $N > 0$ data items\footnote{\small 
Our experiments show that a sampling rate of .1 and $N=4$
makes a good balance between efficiency and quality
(Section~\ref{sec:experiment}).}. We do so in two steps.

\begin{enumerate}
  \item Randomly sample a set $\bar D$ of data items with the 
    given sampling rate.
  \item Check each source $S \in \cal S$. If $S$ provides at most
    $N$ data items, add all of its data items into the sample $\bar D$.
    If $S$ has only $k < N$ data items sampled (\ie, 
    $|\bar D(S) \cap \bar D| < N$), randomly sample $N-k$ data items
    from the rest of $S$'s data items and add them to $\bar D$. 
\end{enumerate}

\eat{
Find out sources that provides values for less than M data items in total, $\cal S_M$, and puts all items covered by $\cal S_M$ into sample set; (2) randomly select $p\%$ of the rest of items as samples; (3) For each source $S$ in $\{\cal S - \cal S_M\}$, if $S$ covers k sample items ($k < M$), randomly select $(M-k)$ items from its non-sample items and add them into the sample set. With {\sc source-base}, the copy detection reduces the computations on sources with a lot of data items but check all the items when a source provides quite few items.
}

\eat{
Our sampling should satisfy four conditions. (1) It should
sample data items whose values have high scores (low probabilities)
and are shared by at least two sources. 
There should be a variety of values provided for
such items, so they often have high information entropy
on value distribution. (2) It should sample
items with high coverage (\ie, provided by a large number of sources).
(3) It should cover a fair number of instances for each source
for accuracy computation. 
(4) The sampling strategy should have some randomness.

Accordingly, we take two samples. The first one mixes high-entropy
items and high-coverage items and we use it for copy detection.
The second one contains high-coverage items and we use it for accuracy
computation. Specifically, given a sample size $Z$, 
we sample in four steps.
\begin{itemize}
  \item Rank the data items in decreasing order of the entropy
    of their values, and choose top-$2Z$ items, denoted by $\bar D_0$.
  \item Rank the data items in decreasing order of their coverage,
    and choose top-$2Z$ items, denoted by $\bar D_0'$.
  \item Randomly choose $Z$ items from $\bar D_0 \cup \bar D_0'$
    and take it as the first sample $\bar D_1$; $\bar D_1$ 
    satisfies conditions (1)(2) and (4).
  \item Initialize $\bar D_2 = \bar D_1 \setminus \bar D_0$,
    and add $Z-|\bar D_2|$ items randomly selected from $\bar D_0'$;
    $\bar D_2$ satisfies conditions (3) and (4).
\end{itemize}

In each round, we (1) do copy detection using $\bar D_1$, 
(2) do truth discovery for both $\bar D_1$ and $\bar D_2$, and
(3) compute source accuracy on $\bar D_2$, and on $\bar D_1$
for sources that do not occur in $\bar D_2$.
}





==> 6_extend.tex <==
Finally, we briefly discuss how to adapt our index for several extensions
of the copy-detection methods described in Section~\ref{sec:overview}.

\smallskip
\noindent
{\bf Coverage and formatting:} \cite{DBH+10a} considers source coverage
and formatting style in addition to value truthfulness for copy detection.
We can still use the same index but when we compute scores for each pair, 
we incorporate coverage and formatting.

\smallskip
\noindent
{\bf Correlated copying:} \cite{BCM+10, DBH+10a} considers correlated
copying, such as copying most values on copied objects, or on copied
attributes. We can use the same index but scan the index in
two passes. The first pass decides for each object and attribute
the probability of it being copied, and the second pass applies the
adjusted selectivity in score computation.

\smallskip
\noindent
{\bf Global detection:} \cite{DBH+10a} distinguishes direct copying
from co-copying and transitive copying by a global-detection phase 
after the iterations. This phase requires computing the probability
of copying conditioned on a given set of copying relationships.
Computation of such conditional probabilities would benefit 
from the index in addition because we can easily see if the copier also
shares the data item with its copied sources according to the
given copying set.

